Explore Aggressively, Update Conservatively: Stochastic Extragradient Methods with Variable Stepsize Scaling

Owing to their stability and convergence speed, extragradient methods have become a staple for solving large-scale saddle-point problems in machine learning. The basic premise of these algorithms is the use of an extrapolation step before performing an update; thanks to this exploration step, extra-gradient methods overcome many of the non-convergence issues that plague gradient descent/ascent schemes. On the other hand, as we show in this paper, running vanilla extragradient with stochastic gradients may jeopardize its convergence, even in simple bilinear models. To overcome this failure, we investigate a double stepsize extragradient algorithm where the exploration step evolves at a more aggressive time-scale compared to the update step. We show that this modification allows the method to converge even with stochastic gradients, and we derive sharp convergence rates under an error bound condition.

==> Figures/EG_StochBilinear.tex <==
%----------------------------------------------------------------------
%%% SETUP
%----------------------------------------------------------------------
% !TEX root = ../Main.tex


\begin{figure}
	\centering
	\makeatletter%
    \if@twocolumn%
        \includegraphics[width=.8\linewidth]{Figures/bilinear_stoch_EG.pdf}
    \else% \@twocolumnfalse
        \includegraphics[width=.4\linewidth]{Figures/bilinear_stoch_EG.pdf}
    \fi
	\caption[.]{
	Behavior of \eqref{eq:EG} and \eqref{eq:DSEG} on Problem~\eqref{eq:planar} with Gaussian oracle noise.
	Even with a vanishing, square-summable stepsize $\current[\step]=1/\run^{0.6}$, the iterates of \eqref{eq:EG} cycle;
	on the other hand, \eqref{eq:DSEG} with $\current[\step]=1/\run^{0.1}$ and $\current[\stepalt]=1/\run^{0.9}$ clearly converges.
	}
	\label{fig:stoch-bilinear}
	\vspace{-2ex}
\end{figure}

==> Sections/Beyond_EG.tex <==
%----------------------------------------------------------------------
%%% BEYOND
%----------------------------------------------------------------------
% !TEX root = ../Main.tex


Given the computational cost of gradient computations, the design of optimization methods solving variational problems with a single oracle call per iteration (instead of the two in \ac{EG}) has attracted a lot of attention in the literature (see \eg \citealp{HIMM19} for a recent overview). Most of these methods are similar to \ac{EG} since they perform a (stochastic) gradient step --the exploration-- step followed by an update.
Therefore, our analysis on \eqref{eq:DSEG} suggests essential modifications in terms of stepsizes that should be carried out in the face of stochasticity.

As an example, consider the \ac{OG} method of \citet{DISZ18}, for which some surprising conclusions can be drawn after applying the double stepsize rule.
The generalized \ac{OG} recursion is commonly stated as follows \citep{MOP20,RYY19}:
%
\begin{equation} \label{eq:OG}
    \tag{OG}
    \update = \current - \current[\stepalt] \current[\svecfield] - \current[\step] (\current[\svecfield]-\last[\svecfield])
\end{equation}
%
where $\current[\step]$ is sometimes called the \emph{optimism} rate. Similarly to our conclusions, it has been empirically observed that taking large optimism rate often yields better convergence in stochastic problems \cite{PDZC19}.


\citet{HIMM19} pointed out that  \ac{OG} is equivalent to the modified Arrow-Hurwitz method introduced by \citet{Pop80} and also referred to as \ac{PEG} by \citet{GBVV+19}. Using a double stepsize policy,  \ac{PEG} becomes:
%
\begin{equation}
\label{eq:DSPEG}
\tag{DSPEG}
\begin{aligned}
\inter
	&= \current - \current[\step] \past[\svecfield],
	\\
\update
	&= \current - \current[\stepalt] \inter[\svecfield].
\end{aligned}
\end{equation}
%
Hence, leading states can be recursively written as
\begin{equation}
    \inter = \past - \pastpast[\stepalt] \past[\svecfield] - \past[\step] \past [\svecfield] + \pastpast[\step]\pastpast[\svecfield]. \notag
\end{equation}
%
We thereby see that \eqref{eq:OG} and \eqref{eq:DSPEG} are almost equivalent and they mostly differ in the choice of vectors that the method outputs at the end.

Taking \eqref{eq:OG} as a starting point, the original \ac{OG} algorithm suggests outputting $\current$ while \ac{PEG} instead looks at $\current+\last[\step]\last[\svecfield]$.
This nuance turns out to be fatal when generalized \ac{OG} is applied to stochastic problems.
By analogy with our analysis for \eqref{eq:DSEG}, we reasonably conjecture that taking $\current[\stepalt]<\current[\step]$ guarantees the convergence of $\current+\last[\step]\last[\svecfield]$, and this may occur even if $\current[\step]$ is set to constant.
Nonetheless, this also implies that if the noise is not vanishing at the solution, $\current$, which corresponds to the exploration state in \ac{PEG}, might exhibit much slower convergence or even not converge at all.

To summarize, when running \eqref{eq:OG} for stochastic problems,
we should look at the \emph{residual iterate} $\current+\last[\step]\last[\svecfield]$ instead of the \emph{optimistic iterate} $\current$.
Interestingly, this conclusion is consistent with the ODE analysis of \ac{OG} by \citet{RYY19}, and explains some experimental results of said work. Furthermore, taking an aggressive exploration step $\current[\step]$ and a more conservative update step $\current[\stepalt]$ may be very beneficial both in theory (for the last iterate convergence and rate) and in practice as confirmed by our experiments.
